Moving object tracking employing rigid body motion on matrix Lie groups

In this paper we propose a novel method for estimating rigid body motion by modeling the object state directly in the space of the rigid body motion group SE(2). It has been recently observed that a noisy manoeuvring object in SE(2) exhibits banana-shaped probability density contours in its pose. For this reason, we propose and investigate two state space models for moving object tracking: (i) a direct product SE(2)xR3 and (ii) a direct product of the two rigid body motion groups SE(2)xSE(2). The first term within these two state space constructions describes the current pose of the rigid body, while the second one employs its second order dynamics, i.e., the velocities. By this, we gain the flexibility of tracking omnidirectional motion in the vein of a constant velocity model, but also accounting for the dynamics in the rotation component. Since the SE(2) group is a matrix Lie group, we solve this problem by using the extended Kalman filter on matrix Lie groups and provide a detailed derivation of the proposed filters. We analyze the performance of the filters on a large number of synthetic trajectories and compare them with (i) the extended Kalman filter based constant velocity and turn rate model and (ii) the linear Kalman filter based constant velocity model. The results show that the proposed filters outperform the other two filters on a wide spectrum of types of motion.

==> figures/bananas.tikz.tex <==
% This file was created by matlab2tikz v0.4.1.
% Copyright (c) 2008--2013, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
% 
% 
\begin{tikzpicture}

\definecolor{tamno_plava}{rgb}{0,0.16,0.3}

\begin{axis}[%
compat=newest,
width=0.35\columnwidth,
clip marker paths=true,
scale only axis,
xmin=-0.322631502763168,
xmax=2.44023813274976,
xlabel={$x$},
ymin=0,
ymax=2.3,
ylabel={$y$},
title={$\sigma_{\omega} =  0^{\circ}$},
axis x line*=bottom,
axis y line*=left
]
  \input{figures/wn_0.tikz.tex}
\end{axis}

%\begin{axis}[%
%compat=newest,
%width=0.3\columnwidth,
%clip marker paths=true,
%scale only axis,
%xmin=0,
%xmax=2.5,
%xlabel={$x$},
%ymin=-0.00594063603117656,
%ymax=2.1,
%ylabel={y},
%title={$\omega{}_\text{n}\text{ =}$},
%axis x line*=bottom,
%axis y line*=left,
%at={(0.35\columnwidth,0)}
%]
%  \input{figures/wn_10.tikz.tex}
%\end{axis}

\begin{axis}[%
compat=newest,
width=0.35\columnwidth,
clip marker paths=true,
scale only axis,
xmin=0,
xmax=2.52562927325619,
xlabel={$x$},
ymin=0,
ymax=2.2,
%ylabel={y},
title={$\sigma_{\omega} = 20^{\circ}$},
axis x line*=bottom,
axis y line*=left,
at={(0.4\columnwidth,0)}
]
  \input{figures/wn_20.tikz.tex}
\end{axis}

\begin{axis}[%
compat=newest,
width=0.35\columnwidth,
clip marker paths=true,
scale only axis,
xmin=-0.4074656210263,
xmax=2.67997973000925,
xlabel={$x$},
ymin=0,
ymax=2.5,
%ylabel={y},
title={$\sigma_{\omega} =  30^{\circ}$},
axis x line*=bottom,
axis y line*=left,
at={(0.8\columnwidth,0)}
]
  \input{figures/wn_30.tikz.tex}
\end{axis}

%\begin{axis}[%
%compat=newest,
%width=0.3\columnwidth,
%clip marker paths=true,
%scale only axis,
%xmin=-0.686289443764278,
%xmax=2.65717823579334,
%xlabel={$x$},
%ymin=0,
%ymax=2.7,
%%ylabel={y},
%title={$\omega{}_\text{n}\text{ =}$},
%axis x line*=bottom,
%axis y line*=left,
%at={(1.45\columnwidth,0)}
%]
%  \input{figures/wn_40.tikz.tex}
%\end{axis}

\begin{axis}[%
compat=newest,
width=0.35\columnwidth,
clip marker paths=true,
scale only axis,
xmin=-0.210031835709318,
xmax=2.59832617268367,
xlabel={$x$},
ymin=0,
ymax=2.3,
%ylabel={y},
title={$\sigma_{\omega} = 60^{\circ}$},
axis x line*=bottom,
axis y line*=left,
at={(1.2\columnwidth,0)}
]
  \input{figures/wn_60.tikz.tex}
\end{axis}

\begin{axis}[%
compat=newest,
width=0.35\columnwidth,
clip marker paths=true,
scale only axis,
xmin=-0.786869217489394,
xmax=3.03413407305892,
xlabel={$x$},
ymin=-0.203117603928398,
ymax=2.9,
%ylabel={y},
title={$\sigma_{\omega} =  90^{\circ}$},
axis x line*=bottom,
axis y line*=left,
at={(1.6\columnwidth,0)}
]
  \input{figures/wn_90.tikz.tex}
\end{axis}

\end{tikzpicture}%


==> figures/stats_SE2R3.tikz.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.6,0}%
\definecolor{mycolor2}{rgb}{0,1,0}%
\definecolor{mycolor3}{rgb}{1,0,0}%
\definecolor{mycolor4}{rgb}{0,0,1}%
%
\begin{tikzpicture}

\begin{axis}[%
compat=newest,
width=0.8\columnwidth,
scale only axis,
xmode=log,
xmin=0.05,
xmax=2.5,
xminorticks=true,
xlabel={$\sigma_{\omega} [^{\circ}]$},
ymin=0.5,
ymax=1.4,
ylabel={position RMSE [m]},
axis background/.style={fill=white}
]
\addplot [color=mycolor1,solid,line width=2pt,forget plot]
  table[row sep=crcr]{%
0	0.588550317921784\\
0.01	0.579492842236024\\
0.025	0.578579008166212\\
0.05	0.576086147823583\\
0.075	0.583358710564417\\
0.1	0.58731871543407\\
0.15	0.581805817033276\\
0.2	0.581036793115776\\
0.25	0.591541793219072\\
0.3	0.589861968725449\\
0.35	0.590594574020807\\
0.4	0.599204892530216\\
0.45	0.602988723975579\\
0.5	0.59833466124959\\
0.55	0.591398193338836\\
0.6	0.602696653323044\\
0.65	0.590262521885066\\
0.7	0.601695877581834\\
0.75	0.595647031360625\\
0.8	0.600962742837316\\
0.9	0.609694862923743\\
1	0.606109611028824\\
1.2	0.600320750964777\\
1.5	0.613870797412106\\
1.8	0.61229501093488\\
2.5	0.62712205742174\\
3	0.624555464875983\\
4	0.640858968433029\\
5	0.666582027792216\\
10	0.941234226233594\\
};
\addplot [color=mycolor1,dashed,draw=none,forget plot,fill=mycolor1,
opacity=0.3,]
  table[row sep=crcr]{%
0	0.609970804718368\\
0.01	0.595846347048647\\
0.025	0.602881335242575\\
0.05	0.597510806178456\\
0.075	0.603691042607972\\
0.1	0.607753034154301\\
0.15	0.60133108832595\\
0.2	0.604222911585658\\
0.25	0.608504185956559\\
0.3	0.609809468418134\\
0.35	0.615298282205044\\
0.4	0.623629178422072\\
0.45	0.624015910837918\\
0.5	0.617896385662355\\
0.55	0.615316721708581\\
0.6	0.623997779871136\\
0.65	0.613008395920398\\
0.7	0.619759491647099\\
0.75	0.624386415607287\\
0.8	0.618905269796053\\
0.9	0.625290305985271\\
1	0.632014458737823\\
1.2	0.619463009993374\\
1.5	0.635718115705647\\
1.8	0.638084238334301\\
2.5	0.666161801229602\\
3	0.659293607262052\\
4	0.669021417811859\\
5	0.734041306155708\\
10	1.95632459120774\\
10	0.87068897253686\\
5	0.629088207920287\\
4	0.621961120259388\\
3	0.597389700479856\\
2.5	0.608367980994796\\
1.8	0.587646153034085\\
1.5	0.593718247224474\\
1.2	0.576508786756961\\
1	0.584350260271789\\
0.9	0.589784692746506\\
0.8	0.571602920710293\\
0.75	0.575613710726287\\
0.7	0.581548918774924\\
0.65	0.571990778648202\\
0.6	0.570771528914006\\
0.55	0.570776868829728\\
0.5	0.580162181872003\\
0.45	0.579100413513711\\
0.4	0.576686154804794\\
0.35	0.57084856105705\\
0.3	0.561515796670823\\
0.25	0.570039024001152\\
0.2	0.559511729322476\\
0.15	0.562267393042033\\
0.1	0.570153533703006\\
0.075	0.562726364830198\\
0.05	0.553415673979568\\
0.025	0.555738701717291\\
0.01	0.555750967550054\\
0	0.566243966487052\\
};
\addplot [color=mycolor2,solid,line width=2pt,forget plot]
  table[row sep=crcr]{%
0	5.46024404339976\\
0.01	2.51490389391315\\
0.025	1.92794017810737\\
0.05	1.30519930776033\\
0.075	1.09768123747069\\
0.1	0.976802423959534\\
0.15	0.839525146057984\\
0.2	0.781222678037897\\
0.25	0.729780175913762\\
0.3	0.729341469992201\\
0.35	0.67359728665791\\
0.4	0.662637848212312\\
0.45	0.67818829359664\\
0.5	0.661959160876905\\
0.55	0.621333273201497\\
0.6	0.631799018245037\\
0.65	0.616160877962414\\
0.7	0.618218833327516\\
0.75	0.629035742377443\\
0.8	0.612648077532903\\
0.9	0.627800880465958\\
1	0.624121055090847\\
1.2	0.605036186303825\\
1.5	0.605710915623184\\
1.8	0.603147607970364\\
2.5	0.605168792646076\\
3	0.597306860443338\\
4	0.597782307440789\\
5	0.595665005346637\\
10	0.616644715033122\\
};
\addplot [color=mycolor2,dashed,draw=none,forget plot,fill=mycolor2,
opacity=0.3,]
  table[row sep=crcr]{%
0	7.86798934492901\\
0.01	3.66507917774299\\
0.025	2.64497146064144\\
0.05	1.78478452941245\\
0.075	1.33222058021467\\
0.1	1.66682073561652\\
0.15	1.01065415444698\\
0.2	0.918428059522013\\
0.25	0.831580295998472\\
0.3	1.0322593944483\\
0.35	0.802537051715482\\
0.4	0.758277042427204\\
0.45	0.766594020419604\\
0.5	0.724771486275069\\
0.55	0.678161461402558\\
0.6	0.700985045689998\\
0.65	0.687372998908901\\
0.7	0.680347734447191\\
0.75	0.729351639436372\\
0.8	0.653182932652503\\
0.9	0.734802546369834\\
1	0.705912722673623\\
1.2	0.636131798891528\\
1.5	0.637044537332081\\
1.8	0.638411388699439\\
2.5	0.637340368291824\\
3	0.644127322309008\\
4	0.620547963405073\\
5	0.625556811277104\\
10	0.658244298584461\\
10	0.593500864754144\\
5	0.571304710341069\\
4	0.578476938265698\\
3	0.574879163173773\\
2.5	0.585730341062071\\
1.8	0.580742669027563\\
1.5	0.587702369311847\\
1.2	0.581540656021006\\
1	0.591619934622135\\
0.9	0.601693675747558\\
0.8	0.579129028577547\\
0.75	0.601139391261319\\
0.7	0.593888248568594\\
0.65	0.592767048431194\\
0.6	0.59540397118056\\
0.55	0.594721872696059\\
0.5	0.627732482736687\\
0.45	0.639534790176097\\
0.4	0.616947370354766\\
0.35	0.64080704386933\\
0.3	0.676964413084162\\
0.25	0.676875841995253\\
0.2	0.720720709018276\\
0.15	0.760381139724117\\
0.1	0.873918822733909\\
0.075	0.968602970937846\\
0.05	1.1518596186903\\
0.025	1.63442191839124\\
0.01	2.1343829613729\\
0	4.53508027015619\\
};
\addplot [color=mycolor3,solid,line width=2pt,forget plot]
  table[row sep=crcr]{%
0	0.588550317900895\\
0.01	0.579469600615603\\
0.025	0.578393786115524\\
0.05	0.57564822026027\\
0.075	0.583304571194284\\
0.1	0.587945501737031\\
0.15	0.58223284220428\\
0.2	0.582295626454571\\
0.25	0.601476257393052\\
0.3	0.606021620257649\\
0.35	0.619040079443398\\
0.4	0.618819579227736\\
0.45	0.651430797018365\\
0.5	0.636713820521267\\
0.55	0.669083451084897\\
0.6	0.685269675152698\\
0.65	0.651946121954418\\
0.7	0.723742625081814\\
0.75	0.688462956368671\\
0.8	0.700052376017939\\
0.9	0.693170991568844\\
1	0.743511033779348\\
1.2	0.802274748207992\\
1.5	0.893983132682555\\
1.8	0.963234047332461\\
2.5	1.06021643434667\\
3	1.23465430010082\\
4	1.20368796991375\\
5	1.43930793479056\\
10	1.32265647723495\\
};
\addplot [color=mycolor3,dashed,draw=none,forget plot,fill=mycolor3,
opacity=0.3]
  table[row sep=crcr]{%
0	0.609970804697507\\
0.01	0.595211011914214\\
0.025	0.602871002621058\\
0.05	0.596665203175602\\
0.075	0.603035121618006\\
0.1	0.608596889723207\\
0.15	0.602346083643845\\
0.2	0.607218617807493\\
0.25	0.627237827142409\\
0.3	0.632379453588315\\
0.35	0.677171925444924\\
0.4	0.651411072972085\\
0.45	0.772337394728863\\
0.5	0.759940210851966\\
0.55	0.84477092940088\\
0.6	0.777149732403996\\
0.65	0.748690475104399\\
0.7	0.896544324830914\\
0.75	0.816450017542259\\
0.8	1.04048314982332\\
0.9	0.764612563998251\\
1	0.981820780452165\\
1.2	1.01617296393542\\
1.5	1.20030594802145\\
1.8	1.36143390112216\\
2.5	1.62221559154315\\
3	1.55603741916735\\
4	1.49184175742497\\
5	1.83547081885815\\
10	1.5791893055908\\
10	1.15321939841844\\
5	1.21389328046656\\
4	1.04209932991263\\
3	1.04821308149586\\
2.5	0.909194011315578\\
1.8	0.84949844422501\\
1.5	0.808889660562868\\
1.2	0.735567529323427\\
1	0.692615934129211\\
0.9	0.651189048450599\\
0.8	0.645800241855201\\
0.75	0.636585899089819\\
0.7	0.671292298507683\\
0.65	0.619125833109996\\
0.6	0.639356109821728\\
0.55	0.629768064713015\\
0.5	0.608784482989103\\
0.45	0.617110246721485\\
0.4	0.596447725931502\\
0.35	0.592654344483099\\
0.3	0.577433156226254\\
0.25	0.578948217855151\\
0.2	0.55958116663215\\
0.15	0.562176006213626\\
0.1	0.569672870179726\\
0.075	0.562115734298539\\
0.05	0.55382533637973\\
0.025	0.556892321814417\\
0.01	0.555560396364097\\
0	0.566243966452069\\
};
\addplot [color=mycolor4,solid,line width=2pt,forget plot]
  table[row sep=crcr]{%
0	0.588550319639421\\
0.01	0.579492566843811\\
0.025	0.578585475341062\\
0.05	0.576097473518517\\
0.075	0.583364474359214\\
0.1	0.587330186850111\\
0.15	0.581798737279695\\
0.2	0.581014613876485\\
0.25	0.591562148597122\\
0.3	0.589941263508347\\
0.35	0.590585377957386\\
0.4	0.599176687123816\\
0.45	0.603174943013829\\
0.5	0.598198940084039\\
0.55	0.591124038666848\\
0.6	0.602743155187258\\
0.65	0.590114514165041\\
0.7	0.601832528676319\\
0.75	0.595263576431017\\
0.8	0.600959115326348\\
0.9	0.609730335086094\\
1	0.605979432832544\\
1.2	0.59993680983298\\
1.5	0.613448753932138\\
1.8	0.611481448031491\\
2.5	0.620801180863481\\
3	0.62035640213872\\
4	0.636132422248766\\
5	0.644614296482939\\
10	0.747357126207248\\
};
\addplot [color=mycolor4,dashed,draw=none,forget plot,fill=mycolor4,
opacity=0.3,]
  table[row sep=crcr]{%
0	0.609970806397165\\
0.01	0.595846061681106\\
0.025	0.602888497586734\\
0.05	0.597510703343466\\
0.075	0.603694860431761\\
0.1	0.607746006658145\\
0.15	0.601810423206429\\
0.2	0.604277625427712\\
0.25	0.608464817743598\\
0.3	0.609797023933002\\
0.35	0.615329844649331\\
0.4	0.623300823946751\\
0.45	0.624315557504687\\
0.5	0.61753315294328\\
0.55	0.614972285915346\\
0.6	0.623877273284297\\
0.65	0.612794710691715\\
0.7	0.619525189549116\\
0.75	0.62405829747867\\
0.8	0.619936480737084\\
0.9	0.624952607379752\\
1	0.630896863541948\\
1.2	0.619116965676498\\
1.5	0.63553633061577\\
1.8	0.63906708327014\\
2.5	0.643450455049576\\
3	0.648536557153826\\
4	0.664134820622667\\
5	0.688243199902917\\
10	1.34357988348908\\
10	0.703643923349729\\
5	0.612741261328466\\
4	0.616742109993401\\
3	0.59362485863678\\
2.5	0.601350724515568\\
1.8	0.587376426625161\\
1.5	0.593473780781618\\
1.2	0.577280542120426\\
1	0.583971153181387\\
0.9	0.589739652081346\\
0.8	0.57254168130726\\
0.75	0.575324146516134\\
0.7	0.581567611171303\\
0.65	0.571406125809555\\
0.6	0.570519751218183\\
0.55	0.570512132846743\\
0.5	0.579812551978173\\
0.45	0.5795212424933\\
0.4	0.576143197105411\\
0.35	0.570908221508376\\
0.3	0.561484149133444\\
0.25	0.570026810971988\\
0.2	0.559457369403008\\
0.15	0.562571488045366\\
0.1	0.570143730238025\\
0.075	0.562708401568803\\
0.05	0.553444735657497\\
0.025	0.55574085834815\\
0.01	0.5557513644951\\
0	0.566243967792381\\
};
\addplot [color=black,solid,line width=2pt,forget plot]
  table[row sep=crcr]{%
0	0.712031806366934\\
0.01	0.70932656187331\\
0.025	0.703600113143179\\
0.05	0.710543672209044\\
0.075	0.701872913213929\\
0.1	0.70901160299898\\
0.15	0.702461906910148\\
0.2	0.713188212822775\\
0.25	0.708299908288995\\
0.3	0.701279641609194\\
0.35	0.710430560019218\\
0.4	0.712958410267859\\
0.45	0.708704418968984\\
0.5	0.714799040273442\\
0.55	0.707733805902575\\
0.6	0.719047991976158\\
0.65	0.703916726141479\\
0.7	0.70603577629631\\
0.75	0.705945392337827\\
0.8	0.705670128544357\\
0.9	0.719098581177752\\
1	0.704748637037751\\
1.2	0.702105833111666\\
1.5	0.703879068798505\\
1.8	0.706215997195164\\
2.5	0.713942475040813\\
3	0.700668636733658\\
4	0.704734395136317\\
5	0.697081235484065\\
10	0.70368230357129\\
};
\addplot [color=black,dashed,draw=none,forget plot,fill=black,
opacity=0.3,]
  table[row sep=crcr]{%
0	0.732158617704798\\
0.01	0.731268650093719\\
0.025	0.730279732872982\\
0.05	0.72192474722556\\
0.075	0.725044186382529\\
0.1	0.727633058908514\\
0.15	0.722420398685349\\
0.2	0.737720662323072\\
0.25	0.731805695541117\\
0.3	0.721174704596865\\
0.35	0.730903228031811\\
0.4	0.736733868719635\\
0.45	0.727016422174361\\
0.5	0.735150855772896\\
0.55	0.733251446942863\\
0.6	0.739136631618117\\
0.65	0.722666521787738\\
0.7	0.733385706496251\\
0.75	0.727029769954139\\
0.8	0.732451861816684\\
0.9	0.738653068588878\\
1	0.726206927285477\\
1.2	0.720674009689942\\
1.5	0.723919551386934\\
1.8	0.728381887115631\\
2.5	0.733780153496744\\
3	0.722880176972616\\
4	0.726862042998287\\
5	0.718719624557456\\
10	0.724682698938751\\
10	0.684794374314046\\
5	0.678234761324035\\
4	0.686759350119677\\
3	0.677419368703751\\
2.5	0.695746814280154\\
1.8	0.682281873891765\\
1.5	0.681286204954922\\
1.2	0.682885796205515\\
1	0.68383529327104\\
0.9	0.698901618608796\\
0.8	0.681403991309514\\
0.75	0.686410154669246\\
0.7	0.686164620764836\\
0.65	0.682086750369922\\
0.6	0.686637511078565\\
0.55	0.687731926137849\\
0.5	0.696244107501885\\
0.45	0.691508737839062\\
0.4	0.699685858790625\\
0.35	0.688035649661239\\
0.3	0.684152524572777\\
0.25	0.683182813890319\\
0.2	0.692641633830811\\
0.15	0.685611332193296\\
0.1	0.688846655104106\\
0.075	0.679272019626737\\
0.05	0.686545855360803\\
0.025	0.682990098207905\\
0.01	0.683354831574902\\
0	0.690124206852129\\
};
\end{axis}
\end{tikzpicture}%


==> figures/w_22.tikz.tex <==
\addplot [
color=gray,
line width=1.0pt,
only marks,
mark=*,
mark options={solid,fill=gray,draw=none}
]
table[row sep=crcr]{
0.501092901209184 0.908837850432579\\
2.28708449316244 1.50474635793948\\
2.31355147988403 2.80867058737619\\
3.51546903080233 3.62560408421703\\
4.70984595444918 4.53004712371237\\
6.69860641846756 5.40059308996208\\
8.35464688078138 6.20038064337282\\
9.78369118109199 6.04525726627613\\
10.278865149437 6.7812688684367\\
11.2631319695977 8.51069950092948\\
12.8200019883005 8.90224879644224\\
15.1122878197322 8.38656900480401\\
15.6068036959484 9.48513534124121\\
15.6715285183204 8.49106483703755\\
17.6804158403947 9.05228039745394\\
18.5572575954918 7.72976827988215\\
19.5388121591276 8.88474470139578\\
20.3887326033059 8.41580684538633\\
21.4526451012317 8.2574085718024\\
23.8695022773228 9.58392700312789\\
23.6054222234302 9.2517196053224\\
25.8673768186986 9.18850604652054\\
24.9412660115921 8.97009798814431\\
26.7453005189583 9.3007770495797\\
27.7189520483276 7.90740596338174\\
29.4747277719647 8.06987217892915\\
30.2202393171989 8.02959938556179\\
30.0697304672315 7.0549502628509\\
31.7672080740273 5.9003417263915\\
33.1920391122312 5.95849034328101\\
32.6581985491164 6.6980654316258\\
33.4779607337063 5.63829744762751\\
34.4765440542256 4.3774456383458\\
34.0254153063416 3.33867418972565\\
36.2452695158239 3.25644279806524\\
36.0401216061798 1.77205496334714\\
35.9937162845744 2.10821316053312\\
36.5302535245061 0.951100239847812\\
36.6809064787014 0.488474332623765\\
37.1450811011154 -0.167453590393199\\
36.3389447025677 -1.93065953401891\\
36.061511927006 -1.25454679152211\\
36.2371996356003 -3.14255089927727\\
36.0532286209947 -3.02970582963989\\
35.4567386004559 -3.38464564752266\\
34.8235444006881 -4.69052775800349\\
34.1442791861511 -5.67770608342905\\
34.5566449984049 -4.43545518795787\\
34.415296718265 -5.43204555777319\\
32.346749347009 -5.92303793398482\\
32.679087028536 -7.86505733161733\\
30.3383707179822 -6.32477378979672\\
30.7601239789777 -7.78656582545355\\
29.3752976055652 -6.05531525325072\\
29.2805330582757 -6.97663231092254\\
28.0004976179508 -8.01376991505597\\
27.6943409354465 -8.14123088659772\\
26.6680810445745 -7.51561285366575\\
25.5459439069479 -7.73228063214892\\
26.0620954719093 -6.40648212547969\\
25.4840157064979 -7.48065951393517\\
22.7957455072525 -6.9987418872598\\
21.8769281235023 -7.74297692198433\\
20.6297233582226 -7.92474754353472\\
21.3997188682273 -7.36593327013648\\
20.5658820047614 -6.35506815488886\\
19.2377619302362 -6.29578058940976\\
19.5939360188942 -6.32679437681069\\
17.4231905132387 -7.33659657714213\\
17.6870312176063 -6.57442248622008\\
15.2965225859094 -7.50397650518577\\
15.5650167578517 -6.86257204285905\\
15.0108218290817 -5.27282293119759\\
14.2598617763127 -7.24370094198482\\
13.1645974395815 -7.43381173295891\\
12.6520808117978 -6.13653179555994\\
11.2068708361208 -6.37820385879028\\
10.2799138141464 -7.24091662717372\\
9.17599468880791 -6.62578481760357\\
9.14600405666897 -7.2024646546393\\
8.40206146333752 -7.55359770527662\\
7.16950788056153 -7.36332273517416\\
6.70593279263543 -7.58459102218792\\
6.10636980853207 -8.40522343463864\\
5.51208228057165 -9.06390501829115\\
5.47112969893447 -8.69175367353286\\
4.25509003159876 -8.63188203918746\\
2.93876972401136 -9.52271106129125\\
3.60345679497551 -10.5971583376168\\
2.42615996519436 -10.9688491579521\\
1.87996518204955 -11.044958009528\\
1.8267001365343 -11.8513749974988\\
1.12756409089016 -12.9488633824351\\
0.925639773280112 -13.6150572067734\\
0.26009778984076 -13.7730352068308\\
-0.0273026732261868 -15.0800020923669\\
1.14415679917453 -16.0789147960681\\
0.428925950227848 -16.2053626555097\\
-0.115841221219679 -18.3759134725253\\
};
%\addlegendentry{Measurements};

\addplot [
color=black,
solid,
line width=2.0pt
]
table[row sep=crcr]{
0 0\\
1.00663212316296 0.993469098150476\\
2.02073845867189 1.97790430863223\\
3.06054634081342 2.90835492917291\\
4.15643057233143 3.7692178320456\\
5.30876147503557 4.59298582214625\\
6.50986288423601 5.33956657269221\\
7.77406176444377 5.99684130351303\\
9.04933550418994 6.56708588646551\\
10.2880753536145 7.07786083738057\\
11.5207510944463 7.51668250079284\\
12.7305343132764 7.913176222201\\
13.9627154740389 8.29955165899817\\
15.1756273619411 8.58325873940437\\
16.3446043921037 8.77741699957095\\
17.4914835560182 8.93279165392451\\
18.5876968768559 9.04135632836292\\
19.6292333172845 9.06253650354988\\
20.6169690535453 9.04160323586581\\
21.6002015992985 9.04599043201181\\
22.635801672562 9.0440791410593\\
23.7279166441026 8.98631508681212\\
24.8677982001318 8.8637137279081\\
26.0241682340042 8.71595715046511\\
27.1736479252516 8.58666254836069\\
28.2824469058105 8.44376461969762\\
29.2901607329826 8.22382075939932\\
30.1854008167919 7.9001482518286\\
31.0154977813767 7.48261365396571\\
31.7819782864133 6.98799620018738\\
32.4897678584533 6.43272692479436\\
33.1132236800626 5.80907088147192\\
33.677726756537 5.1571636120576\\
34.2024946047909 4.46238448688554\\
34.6649717269133 3.79276286970799\\
35.0929078006537 3.14981656558944\\
35.457983800258 2.50611168759404\\
35.78436100569 1.84434632691307\\
36.0698387213224 1.12023665588591\\
36.2870373502844 0.358268061829735\\
36.3912934893963 -0.39951233464521\\
36.3722264342528 -1.12664294472039\\
36.2542375815637 -1.8415150607838\\
36.0586334099472 -2.55368722161476\\
35.7555391957248 -3.21487871089828\\
35.3344623224416 -3.80684631868871\\
34.8440849403839 -4.35176198571916\\
34.3122008257236 -4.84188495021193\\
33.716399773483 -5.2640850652613\\
33.0781743155297 -5.66189531850605\\
32.4242990781835 -6.06172400299954\\
31.7706438642376 -6.42012280917941\\
31.073356032863 -6.74485135886015\\
30.3129832340351 -7.01051332824546\\
29.5557967750896 -7.20356123853977\\
28.8466235469037 -7.34426506079569\\
28.1295938378206 -7.4399037248147\\
27.3890200623704 -7.46258653453997\\
26.6599097799803 -7.40502067622532\\
25.9363230789709 -7.32010413345534\\
25.2100977357909 -7.27165566278481\\
24.5010644804588 -7.25972934964532\\
23.7911490928526 -7.25695665367254\\
23.0532377920584 -7.26339092265911\\
22.2932213992138 -7.24713357047141\\
21.4989394245432 -7.17859062797088\\
20.6922968535728 -7.10459171894215\\
19.8437111012916 -7.0011191140823\\
18.9568882583266 -6.85897489370747\\
18.081826227223 -6.73516514836928\\
17.1961508014257 -6.65805904516862\\
16.3346675362179 -6.5847604051093\\
15.5343948553993 -6.51539720404396\\
14.7089524315592 -6.50211839691085\\
13.8511594448373 -6.55104393668266\\
13.0388969572654 -6.61732649698004\\
12.2692244818001 -6.71391479465746\\
11.5139443497186 -6.85313416922559\\
10.7698953735304 -6.99697320794156\\
9.98993752910782 -7.09026839631309\\
9.16514417655223 -7.13764738810651\\
8.37092806315819 -7.24072476880359\\
7.59807283359605 -7.42691670261229\\
6.83158095495189 -7.66144222314887\\
6.11283555831065 -7.96007466613961\\
5.43544648469122 -8.30791039799528\\
4.7832146729402 -8.65617298128224\\
4.13926918106708 -8.99018044609358\\
3.49085533813204 -9.35324219748824\\
2.89204176371892 -9.80246670458067\\
2.36588844410176 -10.3223301964528\\
1.87851829523566 -10.9401919829141\\
1.47287925499844 -11.6565866360059\\
1.11631017402541 -12.3723784462751\\
0.780156233474553 -13.1093612541111\\
0.484010931731444 -13.9308182976329\\
0.283917954313258 -14.8142699567348\\
0.170277115714508 -15.7483036100665\\
0.110733907847087 -16.7331643557506\\
0.117904902937819 -17.6931564865872\\
};
%\addlegendentry{True};

\addplot [
color=blue,
solid,
line width=2.0pt
]
table[row sep=crcr]{
0 0\\
0.987651165656352 0.997955554090586\\
2.00488041189846 1.954777500273\\
2.8923204756517 2.91733437305347\\
3.7676289697512 3.82749252020737\\
4.7091728144883 4.6983838916731\\
6.03792136689305 5.4989648316256\\
7.57543809322594 6.23450467363243\\
9.17768808894396 6.52248864479371\\
10.4351573173883 6.96246232512109\\
11.5255058980939 7.94323851132246\\
12.7940562785714 8.70362436355939\\
14.5054809350936 8.81649124402286\\
15.7969641674028 9.35198087356676\\
16.6642553941057 9.22865528238292\\
17.8613475234008 9.26753656027365\\
18.8899726687521 8.65257760521028\\
19.8993355046399 8.62969750254878\\
20.8148966452826 8.4042809389497\\
21.7393779951983 8.1669300039362\\
23.1154254903251 8.63590456960335\\
23.9566927948404 8.84006778825078\\
25.335925492351 8.93240429331501\\
25.900901685822 8.92683281463319\\
26.8505349449819 9.0518084824729\\
27.785898026085 8.54522661554806\\
29.0202991175013 8.25077184632973\\
30.1127764251206 8.02276002253869\\
30.6862577770065 7.42497089404994\\
31.6011149374035 6.55304846631518\\
32.7642343877099 6.01810961229646\\
33.3215890008067 5.91994363282072\\
33.9031425558094 5.49093798919886\\
34.5658319306234 4.72796582600243\\
34.7191207297001 3.7971905091592\\
35.6448146687364 3.18929775948016\\
36.100013759952 2.18037518631959\\
36.3570463781964 1.62096792770611\\
36.6567003607283 0.868041998933781\\
36.8608558785462 0.212739645553165\\
37.1252776056831 -0.424485595527773\\
36.8914711222101 -1.4614262476173\\
36.5586049486804 -1.88081122747691\\
36.3538632759101 -2.79996302473995\\
36.0853914207005 -3.35395757119253\\
35.642741696844 -3.78415513642542\\
35.0860475854204 -4.47092052702969\\
34.4328580834047 -5.24984497044245\\
34.0758821318751 -5.28591597110215\\
33.8363569316344 -5.58131381819627\\
32.9488730809674 -5.87870241007687\\
32.5805162828052 -6.79056300523819\\
31.2996112956063 -6.59339881885525\\
30.7299107695004 -7.20011843683716\\
29.7419796988622 -6.70962425258491\\
29.0720289448719 -6.75292184499359\\
28.2829633210062 -7.21071892575745\\
27.6506431314834 -7.56443835362289\\
26.7892490550663 -7.52613676292414\\
25.8349189686186 -7.55812029790994\\
25.4139631820256 -6.99445854258663\\
24.99131424882 -7.00577056239556\\
23.7981562979824 -6.86674244667005\\
22.6818069778289 -7.15704858652621\\
21.4258852048429 -7.41343667186067\\
20.8739008041612 -7.36889899013013\\
20.224167974549 -6.86444688283061\\
19.3709564898482 -6.47429408083822\\
18.9647960977356 -6.19766952663877\\
17.9720239511751 -6.48464754570113\\
17.3911994098845 -6.39454526708975\\
16.1725106311457 -6.76254636995234\\
15.4387634929738 -6.78324106823963\\
14.7974789278697 -6.09710105870949\\
14.1294715598706 -6.437154105567\\
13.3276687913375 -6.80479006999\\
12.5967053755657 -6.53511017286021\\
11.615021074982 -6.43182408201508\\
10.6484050412238 -6.7777459172378\\
9.57334813449305 -6.70353636170075\\
8.86627539632882 -6.94916077836952\\
8.17717800243308 -7.26733345587695\\
7.29050627930523 -7.3965579980033\\
6.55155121285191 -7.57641546507206\\
5.89823572365057 -8.03927724237178\\
5.31296359998042 -8.63598490066492\\
4.93434446213899 -8.90925191074354\\
4.28024519067137 -9.03204401510475\\
3.38668189746586 -9.43141736366633\\
3.08777662930558 -10.1633638151617\\
2.50847826435785 -10.7903019718932\\
1.9360444249366 -11.2259531075456\\
1.58604029369636 -11.8261122871915\\
1.16480101716636 -12.6285676039565\\
0.859629167603991 -13.42679335326\\
0.414614964933047 -13.9906333931936\\
0.0653311607547556 -14.8416822411042\\
0.428609944251725 -15.7530976422224\\
0.415136227062185 -16.4275357035959\\
0.192319355551002 -17.6069715763861\\
};
%\addlegendentry{SE2SE2};

\addplot [
color=green,
solid,
line width=2.0pt
]
table[row sep=crcr]{
0 0\\
0.987831590339036 0.997776589100582\\
2.00244088940325 1.9572940510188\\
2.89463147771207 2.91525541414822\\
3.77268017367198 3.82275835901938\\
4.70792646424962 4.70006439283289\\
5.99599495386774 5.55386627367482\\
7.48393442953501 6.37323538524233\\
9.02650378772957 6.83267853113834\\
10.2577027848029 7.32752224261338\\
11.4029076013494 8.21812935158889\\
12.6834250364169 8.9542816368288\\
14.3346597556004 9.24097205027562\\
15.6353144420875 9.74912734092597\\
16.491699722417 9.69887475318043\\
17.6951101043426 9.77050367214622\\
18.7800834617612 9.28370738517878\\
19.8099518438315 9.26205263925503\\
20.7533087022386 9.04918928181095\\
21.7108130974603 8.80513144037729\\
23.1729291557318 9.08252543960193\\
24.0694095250459 9.18061141258474\\
25.4203189454467 9.2263207893789\\
25.9872888834315 9.17392604316165\\
26.9159125640831 9.24312848008237\\
27.847098021098 8.79043045922751\\
29.0648775224989 8.48854631045043\\
30.1454314792836 8.24734691058847\\
30.7887937887269 7.72468966280077\\
31.7541086323263 6.92095209329771\\
32.8858961938858 6.34584178181615\\
33.442551156064 6.21302851739742\\
34.0311761154704 5.78531552161315\\
34.7231287655407 5.04591146849246\\
34.983845939226 4.1452583209187\\
35.8731772893351 3.47470963006487\\
36.3982640399036 2.4937180344835\\
36.6889622025698 1.92916723545667\\
37.0125429332524 1.16561792841055\\
37.2352865815175 0.493239689155922\\
37.5005949770959 -0.173597658845477\\
37.3517428167808 -1.23463549580609\\
37.0755775713619 -1.72598127807132\\
36.8809544790257 -2.68240894346136\\
36.6386655956304 -3.29070993568108\\
36.2220294194165 -3.7869205018877\\
35.6662094320345 -4.54243049084939\\
34.9985362017188 -5.39318862039576\\
34.6513357243423 -5.5132256390901\\
34.3706668308241 -5.86260017687743\\
33.4499325576473 -6.22851228568949\\
32.8920497366044 -7.13738486494636\\
31.6753097870088 -7.22277509377887\\
30.9414722555437 -7.73182988083912\\
29.9587704603798 -7.43875403269577\\
29.2490482251312 -7.47218454917829\\
28.33653239548 -7.82730506537295\\
27.6154229136708 -8.1153854963908\\
26.7907725456981 -8.0766022922551\\
25.8492117155049 -8.0849021918282\\
25.4081651217485 -7.58471774151214\\
24.9701012404317 -7.55704447764678\\
23.7630766688429 -7.35973201917714\\
22.5824204640213 -7.47249717563088\\
21.3213675675547 -7.63174250186617\\
20.7361599187444 -7.55592741749366\\
20.1145301519754 -7.12829510685884\\
19.2746721542053 -6.77140861675434\\
18.862432597369 -6.51611627662684\\
17.8756519017613 -6.70111148999784\\
17.3028975286456 -6.59596503121214\\
16.106483071223 -6.86158658715219\\
15.3726384134214 -6.85207043808414\\
14.7188573991722 -6.27451107731782\\
14.0534496539911 -6.53425355007877\\
13.2498066796435 -6.82568423474304\\
12.5441520147545 -6.59382973142124\\
11.5808920064109 -6.49586069252381\\
10.6007796789306 -6.73432425815509\\
9.55042754513759 -6.70602096813643\\
8.83745084712321 -6.88909278812518\\
8.13801074085556 -7.15773634317132\\
7.267773880694 -7.29283809828185\\
6.5360739113639 -7.46459864299165\\
5.86553210710675 -7.87955231053427\\
5.2417089465766 -8.42430162965865\\
4.84934868708028 -8.69013535496311\\
4.21020637515501 -8.83884456283431\\
3.33087104519849 -9.23815953404587\\
2.97601552296313 -9.9032864081934\\
2.37527659169207 -10.5182858974026\\
1.79824411167121 -10.9753299298632\\
1.41630554237745 -11.5637185240059\\
0.953007666708706 -12.3583953431351\\
0.597768734135122 -13.154055779024\\
0.157050312194629 -13.7570307264204\\
-0.220229702083632 -14.6147229857238\\
-0.0245297004737192 -15.5604772951668\\
-0.0632699515097228 -16.2527563490987\\
-0.244803734075894 -17.4734212545747\\
};
%\addlegendentry{R2R2};



==> figures/w_37.tikz.tex <==
\addplot [
color=gray,
line width=1.0pt,
only marks,
mark=*,
mark options={solid,fill=gray,draw=none}
]
table[row sep=crcr]{
0.935997459261526 1.34954554622835\\
2.16304009416116 2.32905518439952\\
2.63574211779705 3.50351307863034\\
3.21232030032182 4.05644490320575\\
3.46263632806093 5.45517942094877\\
4.6781221733683 7.30214402344057\\
3.46480876427346 8.77610192416365\\
4.91681786450838 11.062051103395\\
2.49486502344361 13.1584193771433\\
1.47790094614745 14.1128310584217\\
1.40752524743864 14.828995056946\\
-1.54525457740618 14.8059757373285\\
-2.49965002992084 15.0308319754328\\
-4.69840279388993 15.8566444843004\\
-4.76726140489527 14.8127352871688\\
-6.88047245538825 15.5426505674152\\
-8.90045614142551 14.8680096997116\\
-9.25346551675553 13.0393172048014\\
-9.33448232764307 10.4945753446985\\
-9.95777288263088 10.4055569825091\\
-9.96278486010339 8.12741639229779\\
-9.45072000603686 7.24755781642401\\
-9.4607556401234 5.29518593194135\\
-7.24354488913688 3.61163221082651\\
-4.72831995925486 3.59312983850224\\
-3.80892603179526 2.65648578549965\\
-2.35314756233165 2.66718203922225\\
-1.27633660008703 3.35232259276772\\
-0.849550246440001 4.75259520521322\\
2.04447145416077 4.98351095524343\\
3.3270786493951 5.91255045805594\\
3.3503416366305 7.61558321295841\\
3.99775777284035 8.84928959989494\\
5.69658852431789 11.3110927438835\\
6.100253509089 11.9831748255049\\
4.89842694213134 14.6122274514796\\
6.59760713679747 14.0084644563858\\
7.26105292694797 17.5267296838865\\
6.33000695555659 18.0528222325323\\
6.78068141246529 19.0935161576837\\
6.42040249093901 21.1960761254267\\
5.41033245679819 22.3186859974971\\
5.46445382813409 24.3311559270281\\
2.87070280937269 25.6122199153923\\
2.42786249213906 25.7951064380389\\
0.724035037162752 26.1042465175337\\
0.758049370401037 28.3874667029104\\
-0.495926399837243 29.2705407749407\\
-2.47108019420734 30.0447268415518\\
-4.81689658600124 30.4741621569937\\
-5.05703351724621 30.9804551482275\\
-7.62740648864038 31.595030255009\\
-8.77314539389884 32.4401877856859\\
-12.0436566404271 31.5369584220937\\
-13.3279289957355 32.442859611079\\
-14.8022047593712 33.5139604581629\\
-16.5285409843662 33.5515911417791\\
-18.4779758584422 32.5018442143142\\
-20.4200413142973 32.4778253061297\\
-22.0655961039257 33.3165495037998\\
-24.1694452114246 31.6756720721684\\
-26.6857220803608 31.8404215309255\\
-27.8022481494464 30.5612334348673\\
-29.7331345601248 29.9591702401469\\
-31.0180038341667 29.3058728361537\\
-34.3624436828198 28.6237780731883\\
-35.2012984562676 28.628424024037\\
-38.0835509061463 28.9176782635325\\
-38.4396376431728 26.7823465650023\\
-40.6420262969473 27.4086238314985\\
-43.5214125782723 27.0584795500837\\
-45.0639949386372 25.7122008930746\\
-48.184682306937 26.574632007541\\
-49.446163573867 24.7716109227222\\
-50.5048074258021 24.2128410267419\\
-52.7904421865159 21.936766986731\\
-54.3540094700321 20.1997391944948\\
-55.0688208413621 18.738965337482\\
-54.6846798631015 16.5033986450533\\
-53.4677324825488 14.9743082473192\\
-52.1122090258059 14.4739221154063\\
-50.2744437856767 13.2450933658331\\
-48.2896977417036 13.473667482302\\
-45.5835641424232 13.0668206329976\\
-44.5144666460251 15.387057189997\\
-43.2208460821108 16.9379612200765\\
-43.4495609979268 19.2458209944452\\
-44.5815385151723 20.37704674656\\
-45.0309047133348 23.3306985457763\\
-47.8200805507124 23.1346440500679\\
-49.1898310395285 22.8361595231795\\
-51.5236572702789 20.9837251724828\\
-51.2406553182583 20.0129975933828\\
-51.1895130592001 16.6910435252918\\
-49.9991091161312 15.5137606864488\\
-46.7432604222994 15.9797176701964\\
-45.6290388730444 15.4155203157485\\
-44.3162208671492 17.8012461943861\\
-43.6262565458933 19.7536182489058\\
};
%\addlegendentry{Measurements};

\addplot [
color=black,
solid,
line width=2.0pt
]
table[row sep=crcr]{
0 0\\
0.979320215566378 1.01449005627446\\
1.90228023495567 2.09450101123588\\
2.71462619731704 3.33452830451906\\
3.34305186231734 4.72436820492341\\
3.80625426511907 6.19106219132918\\
4.08461669759664 7.73754327164314\\
4.08485910033744 9.31870295001429\\
3.77085933374838 10.8652263543307\\
3.08770922782232 12.2949660131984\\
2.08411455222357 13.5255536733241\\
0.800312554310312 14.5398112884652\\
-0.743944066721894 15.2264735814874\\
-2.399230002591 15.4939031323062\\
-4.03525966463383 15.4426669323443\\
-5.58988966131574 15.1251930627843\\
-7.01985739133573 14.5038278082363\\
-8.23951755084873 13.5186798612831\\
-9.18364710735972 12.2478242468082\\
-9.80168790628925 10.7916330491223\\
-10.0451219527054 9.24927847238915\\
-9.88227891605597 7.71875171462399\\
-9.28300786622805 6.30772070850514\\
-8.29616897338647 5.10212270497959\\
-7.01178423216796 4.12533836405016\\
-5.54592400679122 3.42343095559094\\
-3.99431778740606 3.03787533650505\\
-2.45032508082491 3.07321533688046\\
-1.00274926381678 3.48495088340605\\
0.381168414018269 4.24085229536752\\
1.62329407310939 5.2655334651833\\
2.743445033734 6.45967904593509\\
3.73788226876715 7.74500431357571\\
4.5999096536843 9.07319691720886\\
5.33126373262926 10.4353936034018\\
5.9288219922535 11.866169674181\\
6.37594139195364 13.3879058832331\\
6.65147460504985 14.9300728544243\\
6.78811926226539 16.4887395357378\\
6.76817642600243 18.0621003177795\\
6.54165098926591 19.6020617250612\\
6.13377148121207 21.0841236765371\\
5.54183173822093 22.4742658869345\\
4.73930510453564 23.7649334399158\\
3.78817321694477 24.9929478026043\\
2.7286759413791 26.1404613731251\\
1.51826552437549 27.1862256994298\\
0.121551680014854 28.0897695912651\\
-1.37759864578978 28.8402145475713\\
-2.92514353599219 29.5274094313842\\
-4.50079171775943 30.1927771279051\\
-6.08218329627757 30.7950465209893\\
-7.72178004364062 31.246310616817\\
-9.44952919537921 31.5413632300289\\
-11.2253564324392 31.8225532307045\\
-12.9898187247798 32.1576320057035\\
-14.7500007241176 32.5481264341046\\
-16.571583569089 32.8737054066518\\
-18.4437184878243 33.0117450585586\\
-20.3242391838911 32.9218471740023\\
-22.2089058127278 32.5670029668171\\
-24.1055489169631 32.0327984831645\\
-26.0305562583715 31.4242955829534\\
-27.9165520183947 30.7570718809822\\
-29.7752098666921 30.0605300487883\\
-31.67902804475 29.4074283768499\\
-33.5778752971722 28.8475778121506\\
-35.4485772699213 28.4083303615173\\
-37.3610570183214 28.0704675353457\\
-39.3255940852107 27.7882449753748\\
-41.2808692857934 27.4847991847537\\
-43.2820446963848 27.0701882810814\\
-45.3347352467314 26.500940842897\\
-47.3903626048322 25.87562744199\\
-49.3917015716863 25.107961184773\\
-51.2126359769662 24.0423458825296\\
-52.7637503624838 22.681321021233\\
-53.9694294422267 21.0506843866213\\
-54.647558099406 19.0963641823995\\
-54.5459958629926 17.0281329465825\\
-53.6886697539413 15.1161004005521\\
-52.1993814195347 13.6499797194578\\
-50.3283362680901 12.8247895206591\\
-48.2841556239603 12.7450317663435\\
-46.3078294976724 13.4412583545862\\
-44.6248980601936 14.7637158192707\\
-43.4505107444517 16.6401465509779\\
-43.0208292618944 18.8364275250403\\
-43.5505066429362 21.0486750348847\\
-45.1102792282846 22.7403864360695\\
-47.2989319603774 23.2950446845348\\
-49.4213722139647 22.7422527646264\\
-50.9821902003635 21.1379648131044\\
-51.4636668756163 18.9520256656462\\
-50.7634396238472 16.8445247844563\\
-49.1370443264558 15.4266420641432\\
-47.0037417449783 15.0766240466497\\
-45.0350990414155 15.954388816576\\
-43.847295695624 17.7543914379188\\
-43.8337263826136 19.9560833978202\\
};
%\addlegendentry{True};

\addplot [
color=blue,
solid,
line width=2.0pt
]
table[row sep=crcr]{
0 0\\
0.993908886611075 1.01298848705991\\
1.98794646920413 2.06176457148525\\
2.78170534482325 3.27772357018972\\
3.48776237389802 4.37276992658595\\
3.83416646956697 5.60342268071323\\
4.48286541873855 6.99103344678787\\
3.95710642190977 8.46952666234733\\
4.62356699689704 10.1908394025817\\
3.0174938223596 11.8520330190223\\
1.9073132073701 13.4754774913541\\
1.12769659607225 14.7900969070018\\
-0.896069506623824 14.9925518972523\\
-2.53420217237537 15.0837666337903\\
-4.26945096034837 15.5195104417171\\
-5.51713188936225 14.9861919723492\\
-6.91752103674648 15.0348398515845\\
-8.55434623777634 14.7383299103823\\
-9.55085972951827 13.4071209470876\\
-9.45616516711587 11.412370864951\\
-9.76497421395693 10.05507471841\\
-9.78022996201883 8.42862734741351\\
-9.35224821853363 7.06390950547267\\
-9.15338378205849 5.58424300951008\\
-7.68433941456705 4.16610414629935\\
-5.52908895892597 3.82793874653146\\
-3.97821133837341 3.01755489519455\\
-2.32979813501595 2.78609625772464\\
-0.861891019943665 3.224636559612\\
-0.0517978294693583 4.47142036597171\\
1.4626884582206 5.13094999364526\\
2.86315209103085 5.95254162503954\\
3.53763085140662 7.49625303383907\\
4.04204606015432 8.95098251852208\\
5.11448755913806 10.5918942135914\\
5.8969531131962 12.0159537124026\\
5.25491349055472 14.0205202358192\\
5.84523019459569 15.0305967163558\\
6.67570122691665 16.7600615429498\\
6.58243752132598 18.2835428355567\\
6.72763685306587 19.5821187609618\\
6.53006443871636 21.1433083637002\\
5.73924299262548 22.4450540361271\\
5.39215623585137 24.0547640771399\\
3.62540080961933 25.1004254425169\\
2.32693827742554 25.9039746683734\\
0.75744405842885 26.2436813805093\\
0.186005165137052 27.5464252196846\\
-0.630496973368456 28.7699141164747\\
-2.1330793496377 29.7670544301742\\
-4.09193059800238 30.2392951835444\\
-5.38426447993568 30.9377728476909\\
-7.18501539027123 31.4505732011331\\
-8.70911092734189 32.2216857663603\\
-10.9381106379317 31.6295167379956\\
-12.8760734472162 32.1850656390264\\
-14.5568894732839 33.0859706596108\\
-16.4061842122432 33.5218905872375\\
-18.2774079231844 32.9561398167833\\
-20.197728363798 32.5897247262363\\
-22.0220456359047 32.9530048773947\\
-23.8877975121268 32.0410334815494\\
-26.0692739219784 31.837168951412\\
-27.7960143277227 30.7982231860335\\
-29.6149374503768 29.9636863319507\\
-31.2190421647615 29.1348339370945\\
-33.5027238907974 28.7034110517054\\
-35.3387284259494 28.4176160981903\\
-37.5488062851161 28.6890280349466\\
-38.9802251184403 27.5080958250215\\
-40.7916213032532 27.2201481491039\\
-42.9882498127284 27.0554849747419\\
-44.8552001267532 26.0572904553235\\
-47.2918959915266 26.457825805364\\
-49.213858969368 25.2601602476484\\
-50.8296576068655 24.2966760288888\\
-52.4296361725801 22.5327864004807\\
-53.9940909546876 20.6695550432131\\
-55.0856666791542 18.7842434118698\\
-55.0747323079899 16.5888431947471\\
-53.9862810478135 14.7815002478466\\
-52.2928716522554 13.8539014202556\\
-50.3365924994882 13.217713992145\\
-48.3013006121151 13.439979524468\\
-46.2186954722303 13.4121329249008\\
-44.5884207501708 15.0980881510995\\
-43.3841117547084 16.8807022646622\\
-43.31553655445 19.128376408372\\
-44.3534365246889 20.8527532408569\\
-45.1643967082398 22.7758778445008\\
-47.4718266649483 23.3650712406074\\
-49.4562983521197 23.0275241762134\\
-51.2019090707155 21.3578736801547\\
-51.6942535658292 19.5666438677953\\
-51.1963671162434 17.2519596098132\\
-49.9369687357439 15.6063288591465\\
-47.3157723846735 15.7398619318296\\
-45.5472629437026 15.8941969670485\\
-44.2405068296507 17.6717531319071\\
-43.7739553711741 19.7052327794412\\
};
%\addlegendentry{SE2SE2};

\addplot [
color=green,
solid,
line width=2.0pt
]
table[row sep=crcr]{
0 0\\
0.998438935242831 1.00852547394934\\
2.01025664688137 2.04006169716529\\
2.95496972374228 3.13062804088192\\
3.76168251437106 4.14828280193022\\
4.31904219075632 5.26721651329104\\
4.98966235271566 6.65328537350117\\
4.97079608274185 8.13596495755093\\
5.34203204428419 9.95846802234984\\
4.68809996561954 11.966112056625\\
3.73512463734794 13.6924921067865\\
2.91988724509742 15.0928380608543\\
1.22500511686995 15.9660063373046\\
-0.426594080100927 16.5154709840968\\
-2.44031986328839 17.0445493795882\\
-3.93883379382319 16.9141468363849\\
-5.72479379456835 16.9233439798127\\
-7.68786420508034 16.5756302187085\\
-9.16913897497967 15.5579995613162\\
-10.1532536222518 13.7888043313143\\
-10.9419029733222 12.3605048214492\\
-11.3696841612829 10.4697958670393\\
-11.3465612823622 8.75555860561729\\
-11.183709038 6.83495619786711\\
-10.1434808854957 4.87651398014218\\
-8.34028660302195 3.51524522958522\\
-6.56630460003669 2.31306805927862\\
-4.68628569601095 1.5749900065346\\
-2.90876616022142 1.43663939100873\\
-1.48691090043934 2.00544457659326\\
0.515910301953797 2.67238443580284\\
2.3817410386852 3.61857166307256\\
3.65987578759342 5.02074247064998\\
4.68618903750461 6.56985428041287\\
5.89953320302463 8.62988949139628\\
6.80515757738108 10.4047584052269\\
6.89570754877332 12.6134070241708\\
7.40558226515887 13.9694934905896\\
7.90610401289649 16.1070813971239\\
7.83965808180227 17.778103611049\\
7.83860360674534 19.2441853473374\\
7.62359465407411 20.9273457970189\\
7.02610886332013 22.4302069888483\\
6.5339394466213 24.1076055590632\\
5.19964263980948 25.6602085419629\\
3.9999554511231 26.7158749857782\\
2.49301103874796 27.4291311645433\\
1.39929324777562 28.6015831673523\\
0.196583323401669 29.6527300474435\\
-1.3396067207469 30.5735963441786\\
-3.25777952173585 31.2752385336448\\
-4.69658886088823 31.8424688155534\\
-6.57159619785008 32.3577826233017\\
-8.26853176528951 32.9308199392227\\
-10.5723226583851 32.9331516873375\\
-12.6267937356474 33.1490728337421\\
-14.5284855289501 33.6163614064344\\
-16.3889467302719 33.920781189029\\
-18.2926055112613 33.7081662350816\\
-20.2249201677691 33.4669402511508\\
-22.0696111842512 33.5353669166626\\
-24.007277316608 32.9709393046402\\
-26.1662165812677 32.5653942239503\\
-27.9914474064626 31.7873399712716\\
-29.8395781744062 30.9745541040095\\
-31.4764193917132 30.1379532981046\\
-33.6913223767913 29.2904087256116\\
-35.4645381537152 28.6963218457774\\
-37.6159479206911 28.4148059795784\\
-39.1584496240999 27.5061462080784\\
-40.8810059193588 27.0921595506182\\
-43.0009024079118 26.7264735229016\\
-44.9546064824267 26.0343347723335\\
-47.3371756680757 25.8760704139624\\
-49.3839535639576 25.1815787316936\\
-51.0799802573307 24.5031492152517\\
-52.942251446789 23.2263435968793\\
-54.6848442815286 21.6806920748617\\
-56.0309691574379 20.0471201288997\\
-56.6772267322794 18.0921774191768\\
-56.4933274821759 16.1634385313088\\
-55.6455969184423 14.6537752121352\\
-54.1587836782299 13.230823251845\\
-52.1819686031241 12.4035611224423\\
-49.631218223192 11.8132559698736\\
-47.2900517152552 12.3710298454148\\
-45.1039557498412 13.5276119559433\\
-43.6365433216914 15.371481573145\\
-43.0899523235044 17.2687469170979\\
-43.0212330584566 19.7949751241825\\
-44.1421283924661 21.6240408021953\\
-45.64684677067 22.8080376504691\\
-47.7334811178845 22.9011706163452\\
-49.2702600492388 22.457918590848\\
-50.3930179784599 20.7827411453261\\
-50.7467573444959 18.9594698442258\\
-49.7412344448661 17.6846626988927\\
-48.4567425265091 16.5292790590395\\
-46.9358381834223 16.5595928873185\\
-45.5045037224093 17.3811790820931\\
};
%\addlegendentry{R2R2};



==> figures/w_5.tikz.tex <==
\addplot [
color=gray,
line width=0.5pt,
only marks,
mark=*,
mark options={solid,fill=gray,draw=none}
]
table[row sep=crcr]{
1.32502220678255 1.3823501989587\\
1.79905953337458 3.19988400249687\\
3.58805323827735 1.82925420175013\\
4.25416168737135 3.94118835097617\\
5.23643168759914 4.89200224269945\\
6.16813535225398 5.96980682461595\\
8.09595286941227 7.36262946280532\\
8.12958902725985 8.26242395646825\\
10.2777389262402 8.99163556467003\\
10.7398485301249 9.86678398177175\\
12.4783651175003 10.4596831035108\\
12.8479355583443 11.2222519291128\\
14.4740442891861 13.6849817874465\\
14.9807281694395 14.7243342019115\\
16.3495773538498 15.3289456495634\\
16.2001994797304 16.6773796300153\\
17.7809330231129 18.033185922088\\
18.255307017115 18.6105521101788\\
19.3374727721035 19.4211700902102\\
20.4551576360446 19.8351232136915\\
22.1526035051073 22.0619752736709\\
22.6157314010841 22.1220867637506\\
23.0041124887844 22.6793203001876\\
24.1946131778027 25.0223629335779\\
24.7230238493308 25.8122205857399\\
26.1023673544034 26.7115100652142\\
26.5671359166186 28.0630860496892\\
28.8555548028283 28.984218303129\\
29.0883755686518 30.0431040605708\\
28.5870982384185 31.8619201976213\\
30.3977810241832 32.5069092067725\\
31.752043472108 33.7545621250386\\
31.5558273870769 34.5845222575129\\
32.7505893028648 35.7135155840458\\
33.6569113420147 36.3715721525849\\
33.9425851718998 38.4506911842315\\
34.9007297472358 39.4150829289041\\
35.7625411881508 39.0947698560715\\
36.5200835121204 41.4114303203328\\
37.3363707706818 42.0734641275165\\
38.2805113537384 43.4363977820629\\
39.7533245918254 44.2798424013358\\
40.6796985486706 44.5497759480415\\
39.6880277957273 46.1199083178175\\
40.6835978967655 47.2938807243287\\
42.0213484512925 47.3598803149768\\
41.9651221627546 48.8953234612893\\
43.4248047021261 50.3806221190151\\
43.6298833842441 50.6444009352916\\
43.6677164098091 52.6515859696784\\
44.6633802284229 54.0942816408863\\
46.2016653601713 55.6203110921688\\
46.4643639679755 56.543429771441\\
47.0273253394788 57.933953558018\\
48.1675544589116 58.2524349349622\\
48.0240820337835 60.2330838312561\\
49.6833283417224 61.1996929982257\\
49.2527751909391 61.9971889777046\\
50.6282559988347 62.961416339019\\
51.5503565929998 65.4011672290479\\
52.0762330693948 65.6136167381664\\
52.5348483248106 66.8243580569805\\
51.9952733531515 66.3446948688704\\
53.5040753712056 68.9753784554923\\
52.548616745825 69.9569642510676\\
55.2115742765394 71.7534888012701\\
56.0619521069599 71.9757805553327\\
56.620843968026 73.0070478992248\\
56.5736949308852 73.587513766891\\
58.2743053082059 74.8333650113257\\
57.4499244701845 76.1887246613217\\
58.5974963023988 76.2821534589978\\
59.6952543637368 77.264518832713\\
59.1329863451339 77.5847179828788\\
61.0136380126147 78.2928881794318\\
62.0867253100324 79.367628337163\\
62.2581660977864 79.590587104439\\
62.9471321342031 80.5802148755561\\
64.0067979352673 81.1576014096122\\
63.7971984343322 81.8865461174255\\
65.1155810234251 83.3469218492314\\
66.4166163125676 84.0588074153959\\
66.3749787301707 84.8809228889594\\
67.6588182713428 84.1276336401985\\
67.4013508821489 85.7376068576063\\
68.8739964519644 87.0074546628886\\
70.0300017596358 86.645474878106\\
69.6532619957779 87.0977930887496\\
70.266398586812 87.8578982728604\\
71.5862828855707 88.4613905343064\\
72.5304479506921 89.1481493144912\\
72.9154713758505 90.2324517340575\\
73.595882390991 90.2925911020553\\
74.3412751429985 91.5386672352371\\
75.8346336567511 91.2710197841634\\
76.6930747800778 91.6252689642663\\
76.6634545979138 92.6161009865846\\
78.7670028306798 94.0787181803885\\
79.213211065825 94.0232919332506\\
};
%\addlegendentry{Measurements};

\addplot [
color=black,
solid,
line width=2.0pt
]
table[row sep=crcr]{
0 0\\
1.01274843957834 1.00898170199395\\
2.05520136448984 2.05785904291878\\
3.09053449319081 3.13880679968575\\
4.09710951292004 4.21369448300877\\
5.11076221492612 5.26458206806519\\
6.16019212587659 6.29915555380792\\
7.22967413162154 7.32521433824675\\
8.29538081714376 8.30075997047358\\
9.38612708739787 9.21611134901517\\
10.4685136341929 10.1452837894723\\
11.5583452987444 11.1433550662759\\
12.6676729721188 12.180594003564\\
13.7484872113681 13.238952678568\\
14.8330980899933 14.2805194782529\\
15.899495764393 15.3050058597161\\
16.9399132514822 16.3501568452054\\
17.9132925685803 17.3713537642336\\
18.8039655827598 18.3622899420667\\
19.692947925695 19.4082666181491\\
20.5963250276248 20.5205781593365\\
21.499263203474 21.6044513957636\\
22.3949224724384 22.6398502839475\\
23.311262431236 23.6742464091784\\
24.2495526839186 24.7454017929468\\
25.1666584174473 25.8510487484833\\
26.0937121241671 26.9868364631458\\
27.0277946562736 28.1505208417571\\
27.9169093567609 29.2949761537806\\
28.7653370641886 30.3934568438915\\
29.5749775613145 31.4751795183894\\
30.346120893473 32.5478218501963\\
31.0757346678787 33.6069411179385\\
31.8009500542791 34.6127189517413\\
32.5373401551443 35.5913388104556\\
33.290305608873 36.5987038832557\\
34.1012734273493 37.5999236262845\\
34.9443195709396 38.6245655141632\\
35.7754712656343 39.6742622405464\\
36.588150867176 40.6959483147963\\
37.3518495541582 41.7125387184286\\
38.0671986881231 42.7073613238786\\
38.7850352475479 43.6980173908112\\
39.4917193242628 44.7169038205965\\
40.174781293104 45.782134043837\\
40.8749987665448 46.8839039284133\\
41.5911679358117 47.9700413164508\\
42.2987465122453 49.093086564522\\
43.0191918664983 50.2823623353222\\
43.7424799601078 51.5144381852615\\
44.4446023329177 52.7428547118244\\
45.1308612353678 53.9750542718237\\
45.802883511819 55.217458612618\\
46.4741300602074 56.4246652331532\\
47.1658953385533 57.6202542789578\\
47.8327556696699 58.8023236651903\\
48.4969539491067 59.9803611252583\\
49.1923802579324 61.1726313447785\\
49.8750408070722 62.350620973011\\
50.5340644400096 63.514739539942\\
51.1521603010387 64.6749674213346\\
51.7462336694793 65.804371035484\\
52.3394294521466 66.8633983758855\\
52.9504618216296 67.8858674546788\\
53.5958509422839 68.9205916729058\\
54.2773894578718 69.9659332309292\\
54.9635186675327 70.9857969987025\\
55.5935594068794 71.939849404966\\
56.2314788581949 72.8529892813963\\
56.9241778775232 73.7281026102741\\
57.6409641598088 74.5465374345702\\
58.342937898809 75.3496046606023\\
58.996295856824 76.1355856419406\\
59.6127578700698 76.8931180550599\\
60.2333479547797 77.6554032162614\\
60.8931815109594 78.4312601211887\\
61.559727046866 79.1911588905739\\
62.2249862633314 79.9277907670669\\
62.9170221770438 80.6807153292956\\
63.6298176402695 81.4599828589521\\
64.3432033493881 82.2377411700488\\
65.0814827680945 82.9622922506224\\
65.8564380866699 83.6690325113592\\
66.6125246900142 84.3980344636568\\
67.3385219253919 85.0842178436752\\
68.0268292600705 85.7485930047311\\
68.7025756696648 86.4024926283136\\
69.4389821989974 86.9999519207916\\
70.1854352647983 87.5713898690574\\
70.9015332635324 88.1545812108977\\
71.5749989366587 88.7009594665149\\
72.2443207538652 89.2175634726866\\
72.9751417746855 89.7570354023319\\
73.7433258586826 90.3003428593897\\
74.5793314361155 90.882016611987\\
75.4959572148882 91.5242876733508\\
76.4323149109973 92.1652238224857\\
77.4309833650819 92.7866116389793\\
78.4803646876592 93.3802778326489\\
79.5273750702596 93.9175509932139\\
};
%\addlegendentry{True};

\addplot [
color=blue,
solid,
line width=2.0pt
]
table[row sep=crcr]{
0 0\\
1.00792729641125 1.00932555442422\\
1.99731170877063 2.10999908236833\\
3.08978097837041 2.95181222718231\\
4.15547902633125 3.9288327087867\\
5.21067315024834 4.89978392934131\\
6.22775450949501 5.90552601903088\\
7.55679995611821 7.05295036459949\\
8.4740210330087 8.13958812841262\\
9.80068302677538 9.10911991469729\\
10.8575261268381 10.0360511257108\\
12.1473333800877 10.8311182251883\\
13.1358302095911 11.5853648038247\\
14.3287195202636 12.9201169812744\\
15.2878061650107 14.2106992426279\\
16.3690904067389 15.2967332380189\\
17.006723739529 16.4796948070612\\
17.9185088630683 17.7406859954343\\
18.6618256908303 18.7792860561039\\
19.4945057206858 19.7223115223285\\
20.417226060749 20.4507477183261\\
21.6218351469448 21.6693314848255\\
22.6020146417968 22.5022490241496\\
23.3702244660969 23.2055320078757\\
24.2610268393752 24.4571580430582\\
25.0159802369386 25.5878027776467\\
25.9723441744906 26.6530716799773\\
26.7619467685959 27.826203424495\\
28.0759190083529 28.9272273097688\\
29.0628164680637 30.0178674421616\\
29.515167022459 31.3729938977267\\
30.3827494512717 32.5114348610266\\
31.426868044165 33.6887648163431\\
32.0500481982388 34.7465292680313\\
32.8395293631746 35.8169717757856\\
33.6639648841297 36.7306819535169\\
34.2935411680911 38.0353682338432\\
35.0132861457461 39.2508137733519\\
35.7752321488376 39.9265016934003\\
36.5344103669893 41.126529127221\\
37.3129737727568 42.1556932067136\\
38.1529345600645 43.2984955132984\\
39.2311000247243 44.3442983593928\\
40.2964295069559 45.1051050967234\\
40.6515585537881 46.1135251415501\\
41.1600856891613 47.1820489513111\\
41.9291090681159 47.8985759139827\\
42.408289337022 48.866894723018\\
43.2050356550017 50.0236168140614\\
43.8062549883601 50.8874751024076\\
44.1901265546219 52.1434926014508\\
44.7525882808428 53.5074858075545\\
45.6607469241957 54.9764847948582\\
46.3787920244652 56.300602962803\\
47.0473437285977 57.6681937362747\\
47.8855886814319 58.6786345530734\\
48.3909647586193 60.0050373782343\\
49.2839680642673 61.2194555944453\\
49.7314873452342 62.2826883544702\\
50.4751786619716 63.2872203491932\\
51.2949923914435 64.7826185006104\\
52.0297808618385 65.8653440451095\\
52.6687090132759 66.9741543707522\\
52.8725468242536 67.4992044485143\\
53.4760077250262 68.6899325458483\\
53.520325602105 69.8284020006331\\
54.4306488362743 71.2140776848019\\
55.3821329945146 72.2232151054208\\
56.2467436951751 73.2200065775908\\
56.8129836147226 74.0496858719674\\
57.7686711480156 74.992010617782\\
58.1239041874791 76.0705999163553\\
58.7107230161766 76.8037210373665\\
59.4726416846459 77.5847220542637\\
59.7750221377574 78.1743429596553\\
60.5958954297022 78.7593515791767\\
61.5413637199923 79.4837649876393\\
62.2504099428222 80.0171984924188\\
62.9534683834482 80.6808358866435\\
63.7848012674492 81.3053489820169\\
64.2587745431529 81.9552413771068\\
65.0002672184237 82.8916176373952\\
65.9527606690767 83.7831530567431\\
66.5838142882424 84.6721429616785\\
67.4339693128967 84.9847243979607\\
67.90341397198 85.696629356794\\
68.6940249574038 86.612559836358\\
69.6310506794096 87.0989370299357\\
70.1268761026523 87.5369358969836\\
70.6271554169376 88.0558024052325\\
71.3941032550985 88.5890549911683\\
72.240424248997 89.1671838263412\\
72.9438829287628 89.925867620469\\
73.6370365995827 90.4571852177846\\
74.3456981167245 91.2326295084955\\
75.3369906961963 91.6554406860564\\
76.3200382759096 92.021540593981\\
76.9687599044257 92.5815200090036\\
78.1160350149525 93.4716277279404\\
79.0642567768183 94.0668648109286\\
};
%\addlegendentry{SE2SE2};

\addplot [
color=green,
solid,
line width=2.0pt
]
table[row sep=crcr]{
0 0\\
1.00792730356894 1.00932554728055\\
1.99731331452854 2.10999756035543\\
3.08977696689185 2.95181685448334\\
4.15547246039451 3.92884018071939\\
5.21066461274751 4.89979354964281\\
6.22774773990499 5.90553373161195\\
7.55678634751507 7.05296560329658\\
8.47402702088007 8.1395842249667\\
9.80065890200394 9.10915093488089\\
10.8574952542559 10.0360891491231\\
12.1472554909033 10.8312237666552\\
13.1357341377075 11.5854946666919\\
14.3286946835216 12.92016682675\\
15.2879070471568 14.210641961086\\
16.3692019663101 15.2966615460732\\
17.0070455221521 16.4795016861166\\
17.9189127700716 17.7404394040422\\
18.6623164899571 18.7789877557676\\
19.4949924232704 19.7220009266695\\
20.4176391964631 20.4504816308461\\
21.6221997394439 21.6690867789707\\
22.6022931755355 22.5020846929806\\
23.370451437691 23.2054109018049\\
24.2613429190626 24.4569334238277\\
25.0164068339636 25.5874931190089\\
25.972736189158 26.6527750189769\\
26.7624772971979 27.8258197393971\\
28.076107664469 28.9271582248412\\
29.0630066772704 30.0177789254326\\
29.5161947045199 31.3725748849945\\
30.3837507860614 32.5109890095475\\
31.4276431640362 33.6884024855009\\
32.0510493342719 34.7460260327367\\
32.8405255703924 35.8164222691835\\
33.6648714928108 36.7301438098102\\
34.2946585357753 38.0347225523129\\
35.0144884095815 39.2501114665755\\
35.7763313420213 39.9258457995646\\
36.5355224979252 41.1258270957206\\
37.3140332294363 42.1549956594186\\
38.1539575750804 43.2977969955603\\
39.2318460861814 44.3439178468036\\
40.2969078389831 45.1054854360577\\
40.6521695342861 46.1136799628226\\
41.1608108205881 47.1820527013263\\
41.9297545093827 47.8985174508374\\
42.4089645874802 48.8667235168904\\
43.2056369903773 50.0233705444929\\
43.8068694110857 50.8871654823802\\
44.1911190621337 52.1431595859001\\
44.7536053764088 53.5070401395939\\
45.6601608587334 54.9762732221391\\
46.3782483962294 56.3004283189871\\
47.0473797381507 57.6679162387686\\
47.8845020574692 58.6790449180914\\
48.3912544844869 60.0050721004229\\
49.283530706772 61.2199495299024\\
49.7315726065715 62.2829495558625\\
50.4751885930579 63.2875304493251\\
51.2953039963887 64.7826829783414\\
52.0298979180669 65.8655414845678\\
52.668846403361 66.9742838949774\\
52.8728074252822 67.4992070502945\\
53.4763077989188 68.6898423052454\\
53.5208047970317 69.8280631051802\\
54.4301717306648 71.2135845347626\\
55.3808149505449 72.2235357822123\\
56.2449186974968 73.2213404499624\\
56.8110458187388 74.0517601005444\\
57.7665985000603 74.9945950771406\\
58.1219919987437 76.0730408705692\\
58.7088044291948 76.8061353827684\\
59.470652510735 77.5870487253252\\
59.7737874660741 78.1763030888225\\
60.593564040842 78.7610400364774\\
61.5381381889128 79.4847257866033\\
62.2482715979329 80.0187823279218\\
62.9515762487322 80.6825888300173\\
63.7828153228734 81.3070941656706\\
64.257271374737 81.9572385105751\\
64.998734749743 82.8934103682844\\
65.9509915392459 83.7851199030266\\
66.5826965340867 84.67367077409\\
67.4325528228746 84.9877396527874\\
67.9018738599717 85.6995256489186\\
68.6923495122651 86.6152600146827\\
69.6289477735226 87.1023930359586\\
70.1248290560456 87.5404396641965\\
70.625196889872 88.0590156515739\\
71.3918866092016 88.5920719296912\\
72.2380190518629 89.1700064936591\\
72.9415465087748 89.9284848599543\\
73.6346662017059 90.4598787024816\\
74.3435013022 91.235174972763\\
75.3345867693903 91.6592909150139\\
76.3179240654847 92.0271931741295\\
76.9666088413219 92.5871963259574\\
78.1147914906167 93.4744522741828\\
79.062440547136 94.0706841936871\\
};
%\addlegendentry{R2R2};


==> figures/wn_0.tikz.tex <==
\addplot [
color=red,
mark size=2.0pt,
only marks,
mark=*,
mark options={solid,fill=white!70!black,draw=white!70!black},
forget plot
]
table[row sep=crcr]{
1.01099648186044 1.04831427693648\\
1.04509076408378 1.10605942091616\\
0.943840710127606 0.958495746334641\\
0.967870447173086 0.996052501672144\\
0.973431708240806 0.985694759972762\\
1.03372615842937 1.05184200000628\\
0.984145932804424 1.04667973368493\\
1.02440924066776 1.16330993638194\\
1.01706374672677 0.995823450555865\\
0.973750040304095 1.05038533705806\\
1.00426440343187 0.996583763764032\\
0.976321297086488 0.914823274004786\\
0.955932796700036 1.06279457168543\\
1.00274663403532 1.06992762213717\\
1.01648270309715 0.947104861442447\\
1.01292203950188 1.04458471520074\\
1.02765741226873 1.07292046594477\\
0.950393869168299 0.999415029140118\\
1.00007496085052 0.959183663121604\\
1.01035343324327 0.97777190954337\\
1.02176789813111 1.00085443169784\\
0.968438126196015 0.974983750768635\\
0.947995342169252 1.06327157359245\\
0.913548429154871 0.975587955817602\\
0.973092301414499 1.08886688372134\\
0.962351403842667 0.948343331366858\\
0.970994696830729 1.02086511939265\\
0.971366227244564 1.03296160208389\\
1.00250620250881 1.02742014688101\\
1.03205435872537 1.04733516892344\\
0.971059141266738 1.0028236658557\\
1.05610389352456 1.03879143842299\\
1.06303920286218 0.994604074206737\\
1.0262816301867 1.05759798477789\\
1.04727880996701 1.0753065216659\\
1.06020484676475 0.99940770969576\\
0.929820889726876 1.07710530262482\\
1.01028282692237 0.982689504555308\\
1.01679131679811 1.01661215302443\\
1.0068431462315 1.02888140670291\\
1.07338355627512 1.05652769992117\\
1.00621668458176 1.08897155684321\\
1.0428996235864 0.956082260935047\\
1.04313913512634 1.03241525720245\\
0.968340430625759 1.05089947091465\\
0.997626295575809 1.0844572734646\\
0.887446084885169 1.01782445648073\\
0.98502244804932 0.968287570337989\\
1.06205350660537 1.02776402712327\\
1.02290816695439 1.03419919950965\\
};
\addplot [
color=blue,
solid,
line width=2.0pt,
forget plot
]
table[row sep=crcr]{
0 0\\
0.991074805235027 1.02538629151138\\
};
\addplot [
color=red,
mark size=2.0pt,
only marks,
mark=*,
mark options={solid,fill=white!70!black,draw=white!70!black},
forget plot
]
table[row sep=crcr]{
1.96881790699209 2.07656033835311\\
1.91206226272202 2.02257134429888\\
1.97069384173876 2.03965134336709\\
2.01087396126988 2.01847279731066\\
1.90882909404053 2.08033775898005\\
2.00735315128211 2.02184049387404\\
1.96605900281356 2.14575655764224\\
1.94636520551199 2.06471226249713\\
2.04517547920844 2.0506038902413\\
1.96316226449629 2.13333404514524\\
1.98142863387962 2.1654291500913\\
1.98617623099203 2.03256719885975\\
1.95600742859333 2.10853972918494\\
2.01317150295686 2.02260500160786\\
1.94550226035646 2.06151171969372\\
1.99209416882164 2.12573759251601\\
1.93358010949984 2.12269977725941\\
2.01321388942126 2.10614074570846\\
1.90223732443111 2.06597706994388\\
1.97824198756418 2.1199767048755\\
2.00582520410342 2.08508539408829\\
1.95696954356707 2.08121626633209\\
1.9701480101074 2.11243826277768\\
1.98277094540847 2.03941795577831\\
1.8749553039173 1.97838266389857\\
1.96575341251207 1.97774546904127\\
1.96887833116178 2.09152817918548\\
2.02657400359807 2.09280595061494\\
2.02561225723823 2.17910201897713\\
1.96119820123602 2.12808263382366\\
1.89907043041851 2.0708344790086\\
1.9805140672234 2.02025460386183\\
1.93925000797227 2.12391159708987\\
2.00569462449054 2.10608462655703\\
1.8741844688406 2.09430578813135\\
1.93559456835171 2.07531300109899\\
2.058291155621 2.07463041362412\\
1.92083390421042 2.03939035665011\\
2.00965369451656 2.10651821734695\\
2.11760662998659 2.12211564510151\\
2.06903361019675 1.95337449579232\\
1.97199041328384 2.08615567692288\\
1.99969275732367 1.96530293474939\\
1.99516988627689 2.07410920426399\\
1.93503953451673 2.1036350772235\\
1.89026646841748 2.06064744458525\\
1.92199485630723 2.10140880015513\\
1.96048790409302 2.04877207870451\\
2.03187455945162 2.06670580893646\\
2.04885242065525 2.16582241064895\\
};
\addplot [
color=blue,
solid,
line width=2.0pt,
forget plot
]
table[row sep=crcr]{
0 0\\
0.991074805235027 1.02538629151138\\
1.95693204282484 2.04701812858992\\
};


==> figures/wn_20.tikz.tex <==
\addplot [
color=red,
mark size=2.0pt,
only marks,
mark=*,
mark options={solid,fill=white!70!black,draw=white!70!black},
forget plot
]
table[row sep=crcr]{
1.19221340429897 0.790337882796416\\
1.07909585746574 0.940011316634973\\
0.99645856717296 1.07151605409095\\
1.01398266897619 0.924959473594203\\
0.880250835096034 1.03108949433066\\
0.885114660460474 0.913456845140155\\
0.970380361241813 0.998714986853936\\
1.19003270204154 0.877278584793885\\
0.991202103116575 0.928278214953626\\
0.790452172027969 1.09986848388516\\
0.958147990720413 1.01653423436044\\
0.873724236492199 0.979292929366254\\
0.918803552113754 1.03553814677274\\
0.986998546700785 1.01652815624396\\
0.98279175559456 0.897250330854334\\
0.903606812376248 1.00822691791466\\
0.979444924679689 0.962349029751288\\
0.884489773240626 1.06012183878335\\
1.01132093717385 0.972343792196554\\
1.03915516717357 0.945993449802392\\
1.06298960050025 0.930575111954751\\
0.92767868173358 1.07127123445394\\
1.06787899049013 1.00460564165873\\
0.969800645787118 0.990028807854316\\
1.05469150649777 0.998983740100502\\
0.957353071342752 1.00491694491117\\
0.980512206528576 1.07591527797545\\
0.983766207101006 1.05003012835795\\
0.886351999950884 1.06369156816813\\
1.11314417819657 0.994089370676592\\
0.887270080927191 1.06167571049384\\
0.673946732742658 1.13716237229562\\
1.07037090130742 0.875916788478787\\
0.883377566425232 0.99899534212303\\
0.878285304616438 1.07476152680844\\
0.918239380579278 1.07079266626237\\
1.11106141144188 0.978495215734436\\
1.07106189805736 0.887375088041389\\
1.00624425476698 1.06966027894867\\
1.03649487432112 0.984366009091178\\
1.15668304615682 0.709011370376592\\
0.989035018836609 1.13758727254487\\
1.16789775719586 0.880934853002117\\
0.85843165865708 1.04567597027099\\
1.08354400906565 0.882498589978041\\
1.04461098095859 0.855746152959564\\
0.990776713405841 1.12812961220387\\
0.935309190189176 1.1145848177396\\
0.940558463287099 0.8435080631885\\
1.0084770671867 0.86130396500441\\
};
\addplot [
color=blue,
solid,
line width=2.0pt,
forget plot
]
table[row sep=crcr]{
0 0\\
1.00774679032447 1.00231518067713\\
};
\addplot [
color=red,
mark size=2.0pt,
only marks,
mark=*,
mark options={solid,fill=white!70!black,draw=white!70!black},
forget plot
]
table[row sep=crcr]{
2.12734965903831 1.8970388089959\\
2.10218463127188 1.90861711094756\\
2.04169818806789 1.94019667644149\\
1.94468017939561 2.02082848391402\\
2.09893757895829 1.95208441315194\\
2.06892309533112 1.99767539962668\\
2.14888281855923 1.98090915319997\\
1.95971157309541 2.0213284007393\\
2.31006544295021 1.70825431398661\\
2.17913514204186 1.90602495515226\\
2.39192571551268 1.46250219531546\\
2.13553520931424 1.74989619993944\\
2.19890799414234 1.83297969638512\\
2.21284007878211 1.81238117778389\\
2.09463119947147 1.86880375099144\\
2.00321854251268 1.9757822651408\\
2.13201502401858 1.83790834875494\\
2.10951979027233 1.94408054570935\\
2.07720692734446 1.96217747609893\\
2.25103341298803 1.71158494714246\\
2.1029124152703 1.98840349576251\\
2.20704809682239 1.79339552506521\\
2.2431740308801 1.86945556027999\\
2.15144959570979 1.8738896543168\\
1.97112255513842 2.06603638735832\\
2.13769229428713 1.86763456450429\\
2.3102956808421 1.81649076688784\\
2.10012523744842 1.93191808812761\\
2.25252652823999 1.67407501845303\\
2.09466707746199 1.8568405178386\\
2.164361877764 1.89761270632986\\
2.18081216626117 1.91084244930101\\
1.97617817129369 2.09744153928848\\
2.14887493994276 1.93436867700001\\
2.22291948590261 1.81796199213929\\
2.09348424642492 1.96847996868088\\
2.13994732479487 1.90712219416189\\
2.09246802929097 1.94551978477902\\
1.92885820464484 2.00542218997438\\
2.08106572247817 1.88239684930325\\
2.00571208834001 2.02507680270348\\
2.26765452091823 1.82422225422681\\
2.09035573469278 1.8966314221847\\
2.08666451335252 1.78988680155479\\
2.08084604498879 1.82338525067497\\
2.04037689987425 1.97394783871401\\
2.11403145746815 1.81172329834869\\
2.01384847879983 1.91792533507661\\
1.98885171036918 1.99423042081416\\
2.17609487059978 1.73471345706059\\
};
\addplot [
color=blue,
solid,
line width=2.0pt,
forget plot
]
table[row sep=crcr]{
0 0\\
1.00774679032447 1.00231518067713\\
2.16928008733268 1.77839122340965\\
};


==> figures/wn_30.tikz.tex <==
\addplot [
color=red,
mark size=2.0pt,
only marks,
mark=*,
mark options={solid,fill=white!70!black,draw=white!70!black},
forget plot
]
table[row sep=crcr]{
1.26100315912111 0.779604620024362\\
0.730565551021322 1.13786595975638\\
1.09601866902811 0.984449549529155\\
1.21631375342272 0.684168116729574\\
1.1082440304443 0.894418542614522\\
0.904125686866333 1.02420976907341\\
0.986321428529538 0.992425934587255\\
1.08462389612762 0.840717654119427\\
1.04882044130383 0.859481525131355\\
1.14202781818143 0.674876018705037\\
0.964792366256444 0.90912378379366\\
0.895881582442882 1.08288829919105\\
0.984837389302097 1.10504227309805\\
1.13406610119201 0.849343169674483\\
0.670865827105875 1.10570752758377\\
0.925874466886196 1.03390127450399\\
1.06900112259533 0.950914379715357\\
0.999693787115168 1.01612487292047\\
1.14662223295408 0.943594120433126\\
1.19631818537217 0.806105723491429\\
1.01430610086604 1.078851268342\\
0.642459059495702 1.28159905739407\\
1.04704016636943 0.972484686698292\\
1.2101390373664 0.635935969949236\\
0.882968961388039 1.08465694517491\\
0.906076054665097 1.04966152373154\\
1.16558910386701 0.870603750759747\\
0.925252905994989 0.967341133958981\\
1.08246977414949 0.933436645012272\\
1.10075423956403 0.714497140615939\\
1.08306951171236 0.90034280517034\\
0.834330314404787 1.03545736140905\\
0.904298745940245 1.1033964332119\\
1.222660186722 0.704969862379327\\
0.860438511885249 1.09946174679725\\
0.938486279280959 0.971420869296317\\
1.10600548015786 0.880104509415687\\
1.16489739757492 0.834531739119913\\
0.502254687564949 1.16860989535816\\
1.04024041218359 1.00482912517858\\
1.13508538853635 0.867144060613377\\
0.920766426919281 1.09468516901258\\
1.06322414046622 0.933135644513208\\
1.0000635252978 1.07256234574166\\
1.01518869225424 0.839462280790168\\
0.941252943513715 0.987886950319461\\
1.09891996942612 0.955716763960178\\
1.0547349311717 0.879224236455164\\
1.01936937490414 1.06993122103423\\
1.23174630473692 0.753742707977379\\
};
\addplot [
color=blue,
solid,
line width=2.0pt,
forget plot
]
table[row sep=crcr]{
0 0\\
1.01143185186296 1.03961479675593\\
};
\addplot [
color=red,
mark size=2.0pt,
only marks,
mark=*,
mark options={solid,fill=white!70!black,draw=white!70!black},
forget plot
]
table[row sep=crcr]{
2.14819806389058 2.0718104963285\\
2.11478098576158 2.01203756435246\\
2.09160199843662 2.15998954183335\\
2.21152190341943 1.86275966990032\\
2.1542967909457 1.89098114473651\\
1.97293815972623 2.10597565061307\\
2.08706851557626 2.08750591115463\\
2.24622703051058 1.98439906831062\\
2.04730248260946 2.10131029048121\\
2.00108911621364 2.13922803208465\\
2.01913560477519 2.18248661389071\\
1.97166689857804 2.19567181720137\\
2.13104309696965 1.87947505292752\\
2.02007005742048 2.11819140357097\\
2.12254347495213 2.07811846822918\\
2.09932056305307 2.08158568207517\\
2.11519184400629 2.04179190156836\\
2.10188836978799 2.13904219540083\\
1.81821845803969 2.19948728597361\\
1.96367494591286 2.14306095760724\\
2.18545731887231 1.99857878763534\\
2.01876581948966 2.11287219036747\\
2.01461465507126 2.12023074070969\\
2.18193773319686 2.09530307460453\\
1.9414642230766 2.2110163070652\\
2.27251410898295 1.87583314798056\\
2.03854061912995 2.09664045064077\\
1.88011521607444 2.20224516638508\\
2.19311157430628 1.96678168285508\\
2.09383037575715 2.03430754714342\\
2.16381121142761 1.9855437806261\\
1.90073451514252 2.20591653681414\\
1.62715533522019 2.28551364588935\\
1.93841727980216 2.14120749948317\\
1.78667800984558 2.43509802686513\\
1.76407824247628 2.31809048028754\\
2.05859982487669 1.96864070412985\\
1.97028754927731 2.14570794618342\\
1.90094109852578 2.22472645615139\\
1.93235471468565 2.22750847954221\\
1.95690837115921 2.17281298477844\\
1.8079324091219 2.19532100724766\\
2.00771148049953 2.154051159087\\
2.22512461704373 1.74657264026784\\
1.83624705801728 2.18112792086066\\
2.07786411375767 2.07611652292371\\
2.13888651993075 2.06628329701394\\
2.0459961131501 2.07274236252349\\
1.81915029926049 2.20645504311076\\
2.06631677160156 2.13999979845686\\
};
\addplot [
color=blue,
solid,
line width=2.0pt,
forget plot
]
table[row sep=crcr]{
0 0\\
1.01143185186296 1.03961479675593\\
2.0167183927977 2.23445788647397\\
};


==> figures/wn_60.tikz.tex <==
\addplot [
color=red,
mark size=2.0pt,
only marks,
mark=*,
mark options={solid,fill=white!70!black,draw=white!70!black},
forget plot
]
table[row sep=crcr]{
1.03149873615913 0.822686432589824\\
0.815462868091912 1.0656149788721\\
1.37529815849496 0.479865226714301\\
0.560607671227242 1.25556066846897\\
0.0827095279949904 1.26069628651929\\
0.950689916009841 1.16290562937762\\
1.20655283406771 0.906842149374637\\
0.744192292856728 1.17076151294396\\
0.401264382281603 1.3599223433852\\
1.20249700404846 0.596443223557167\\
0.951362340646787 1.07649690209774\\
0.907836055433428 1.10617280063439\\
1.06252744977429 1.02221220128364\\
0.750013064648206 1.14432345463156\\
0.775205242953268 1.21378464268506\\
1.21754200442641 0.794353493527991\\
1.25217622118063 0.694889662799855\\
1.16796965282965 0.903524673897348\\
0.42541641076515 1.33926879882057\\
0.980634818206694 1.01817409435968\\
1.16753567790542 0.905913459647734\\
1.2469159059455 0.686924051740198\\
1.13316117376063 0.69543015327726\\
1.2874322061931 0.261306428826246\\
1.18780805764659 0.638144083252984\\
1.02736336825492 0.961314783007147\\
1.14462259078997 0.8409931184873\\
1.33435052211062 0.673165025473411\\
1.25408915467399 0.316867121969653\\
1.14564877027977 0.618560115676605\\
1.02934735064434 0.913200096140096\\
0.728681733899618 1.24235108537771\\
1.00351691353032 0.998419548998644\\
1.17932648068999 0.918926022004595\\
1.00760685350677 1.13596752009891\\
0.451839487843815 1.29083884097791\\
0.86833499836903 1.03593724465095\\
0.853823621034233 1.17519039193704\\
0.71388742771379 1.26197910611199\\
0.856046015989273 1.1598868115906\\
1.15499503557811 0.897156186927248\\
1.15131955552574 0.641234000192426\\
0.661531395236729 1.27025373748779\\
0.757464901225746 1.2635890780589\\
0.807781024164329 1.08648849339008\\
1.26855302317213 0.591521876049331\\
1.13263218350086 0.649034113825067\\
1.27731893801722 0.654039325631034\\
1.29746520311037 0.652635798269867\\
1.05797587344323 0.858693456732465\\
};
\addplot [
color=blue,
solid,
line width=2.0pt,
forget plot
]
table[row sep=crcr]{
0 0\\
1.0164259527376 0.967123780382973\\
};
\addplot [
color=red,
mark size=2.0pt,
only marks,
mark=*,
mark options={solid,fill=white!70!black,draw=white!70!black},
forget plot
]
table[row sep=crcr]{
2.20694093523606 1.72541578602153\\
2.32627112250487 1.2323714900078\\
2.06441313970087 1.86580402468972\\
2.24640941864652 1.6197184717098\\
2.12211183292243 1.70462312946389\\
2.33067440326657 1.19505929619516\\
2.14368226297298 1.83399934208382\\
2.1257877409377 1.79603291172192\\
1.32329465925673 2.20062216646558\\
2.20099351340242 1.64121668556153\\
1.95484076275828 1.99602008772671\\
2.26361013768913 1.55204720704111\\
2.19983828534419 1.79590435476995\\
1.63882949046835 2.2149791388777\\
1.76127379879704 2.15787698971467\\
2.1436933058847 1.8688818059137\\
2.25980408349633 1.4115442718367\\
2.09875652255611 1.97842837071394\\
2.04456688279604 1.88322722589703\\
1.90245918416683 2.0992553971464\\
2.30468239034898 0.935532309616977\\
2.2385076044447 1.54165933041267\\
1.88422526845475 2.01699398311493\\
2.02623893452761 1.88479436202116\\
2.21244008037652 1.63361882808517\\
1.91839809001837 1.90942808397693\\
2.0405103318642 1.93430248075691\\
2.22154917121725 1.73977953432257\\
2.38829433697435 1.05208029656945\\
2.09811292802154 1.97812616290786\\
2.27108793166489 1.51007893806058\\
2.14779801289089 1.72683192307299\\
2.34552017061331 1.06144443150323\\
2.16392635335037 1.69555258949766\\
2.14561303505002 1.71714510924126\\
1.85125830876111 2.02824710210549\\
2.14672139062791 1.73275582166927\\
1.94248474614759 2.06180395099776\\
1.8315996966352 2.08863622956294\\
1.92817773150143 1.89016242519969\\
2.16015985380241 1.81109920765527\\
2.25784211082871 1.72457832403092\\
1.9520585718723 2.00951060207936\\
2.30966361265857 1.48257883393619\\
1.82673716603746 2.05770151274534\\
1.96752506545612 1.92845997540326\\
2.22481064371768 1.67976388457852\\
2.03270644505695 1.90485917340136\\
2.21592748534818 1.51492385576205\\
2.19828941255672 1.76189424805678\\
};
\addplot [
color=blue,
solid,
line width=2.0pt,
forget plot
]
table[row sep=crcr]{
0 0\\
1.0164259527376 0.967123780382973\\
2.24765716202173 1.51259350298264\\
};


==> figures/wn_90.tikz.tex <==
\addplot [
color=red,
mark size=2.0pt,
only marks,
mark=*,
mark options={solid,fill=white!70!black,draw=white!70!black},
forget plot
]
table[row sep=crcr]{
-0.211599121218367 1.20230656995068\\
1.23963337866882 0.496118856670396\\
1.10301582075222 0.814870871880034\\
1.01412343751481 1.03223907769217\\
0.425434993701463 1.35306091528471\\
0.574579748779789 1.24760148379249\\
1.01340096153176 0.903069230980964\\
1.02641150760545 0.958414886356431\\
1.20430561186871 0.527147796921165\\
1.27293241113687 0.233968301419485\\
0.794609515867836 1.26647101273635\\
0.604990594345694 1.20631318954598\\
-0.0191237438631662 1.31338989985286\\
1.12989811138205 0.765598044725349\\
1.17992459555613 0.690869483703105\\
1.11015867909403 0.692848422605446\\
0.872374355330296 1.06944424749264\\
1.1728500235828 0.811416972395433\\
0.746586392748129 1.16054054004552\\
1.09448589472147 0.919527101409181\\
1.08244803886281 0.862977348042145\\
1.33487622323591 0.642079649206119\\
1.33512594044869 0.548475162410722\\
0.967512995702748 0.99864362627634\\
1.29922528587722 0.551604932636253\\
1.26661893898528 0.199458568748857\\
0.993972308511101 0.926966488355612\\
0.938383962453368 1.07142633702642\\
0.522076877674097 1.25310511399838\\
1.32577661887076 0.527873444612323\\
1.37185442916914 0.360548873799603\\
0.944192509621526 1.01729278436749\\
1.24786657850153 -0.203117603928398\\
0.918818683796872 1.08106548364073\\
0.619779646177915 1.27308726639926\\
0.951335050249284 1.03626765516515\\
0.709284039144508 1.24538934541728\\
0.959319751804085 1.00911537541492\\
1.28851342260421 0.458478906673335\\
0.946763732921707 1.0071287149739\\
0.954770101497704 0.975762770454373\\
0.591559592255917 1.24108234026486\\
0.999869226663985 1.05324698501819\\
0.26303057705894 1.32444995687084\\
1.03252831474631 1.05999851944457\\
0.722358318299487 1.12848518468686\\
1.24788796999581 0.648311057452196\\
0.906337570813711 1.18934718146975\\
1.04695429444102 0.950890393400265\\
1.08264998082887 0.91614538421568\\
};
\addplot [
color=blue,
solid,
line width=2.0pt,
forget plot
]
table[row sep=crcr]{
0 0\\
0.99953442988279 1.16810460256773\\
};
\addplot [
color=red,
mark size=2.0pt,
only marks,
mark=*,
mark options={solid,fill=white!70!black,draw=white!70!black},
forget plot
]
table[row sep=crcr]{
1.68764179353532 2.59054486022418\\
1.34542588158551 2.728425225283\\
2.07682904471175 2.39997111769219\\
1.51761968872437 2.76297218396127\\
2.10435466955878 2.31530056550111\\
1.64845459378159 2.70451460100109\\
1.34575411609512 2.7547778992186\\
0.43566206068084 2.35938366208103\\
1.98516131228171 2.47750835718571\\
1.46361712476604 2.74435033073779\\
1.9392119723763 2.5253829787931\\
1.29485356673303 2.73236227973235\\
1.89173664251969 2.56953250100308\\
0.838652705628391 2.62889309208912\\
0.576099039999325 2.5380971680708\\
1.90651643012298 2.56321293717498\\
1.63082267277764 2.63230157048871\\
1.25332764898016 2.70233005234103\\
1.55051695166857 2.78684873946424\\
2.19241914543316 2.36067042356808\\
1.88875335206523 2.45208305216713\\
2.36755623814483 2.00025287286211\\
1.25299385579887 2.75847860756033\\
1.75477588178467 2.68952210711826\\
1.93751051432145 2.56791132423775\\
1.06230781227041 2.77057542964264\\
1.64349087222768 2.67367250312798\\
1.10925605959342 2.81054466877825\\
2.00301056619039 2.47236191764079\\
1.4027302630979 2.64416655224368\\
2.35693510464705 2.00040703310145\\
1.07009551086814 2.76416671400281\\
2.05464550053122 2.4716675719291\\
2.32031616412028 2.08621624256047\\
1.72040174124378 2.67340824050313\\
2.24020321324569 2.37919391780007\\
0.927499332548025 2.64115783165186\\
1.137227252256 2.7187537654398\\
2.21895821756623 2.41266341320191\\
0.57450804137843 2.55381486205459\\
0.792275380248889 2.687136134397\\
1.16994214760022 2.78628857417815\\
1.04086431617611 2.65680711750533\\
1.39052761353065 2.73836274570286\\
0.800406773593074 2.57786073066516\\
2.45886397678789 1.76893862986377\\
1.66761083811077 2.76505587474565\\
1.22929617478667 2.7538891794891\\
1.81425523790657 2.62608685662838\\
2.19699841419428 2.34835542194615\\
};
\addplot [
color=blue,
solid,
line width=2.0pt,
forget plot
]
table[row sep=crcr]{
0 0\\
0.99953442988279 1.16810460256773\\
1.22070370421884 2.72747229021865\\
};

